Feature-Driven Strategies for Trading Wind Power and Hydrogen

This paper develops a feature-driven model for hybrid power plants, enabling them to exploit available contextual information such as historical forecasts of wind power, and make optimal wind power and hydrogen trading decisions in the day-ahead stage. For that, we develop different variations of feature-driven linear policies, including a variation where policies depend on price domains, resulting in a price-quantity bidding curve. In addition, we propose a real-time adjustment strategy for hydrogen production. Our numerical results show that the final profit obtained from our proposed feature-driven trading mechanism in the day-ahead stage together with the real-time adjustment strategy is very close to that in an ideal benchmark with perfect information.

==> reference.tex <==
@article{miguel,
  title={Online decision making for trading wind energy},
  author={M. A. Muñoz and P. Pinson and J.~Kazempour},
  journal={Computational Management Science},
  volume={20},
  pages={1--31},
  year={2023}
}


@article{kuhn,
  title={The decision rule approach to optimization under uncertainty: Methodology and applications},
  author={A. Georghiou and D. Kuhn and W. Wiesemann},
  journal={Computational Management Science},
  volume={16},
  number={4},
  pages={545--576},
  year={2019}
}

@misc{entso,
  title={{ENTSO}-e transparency platform},
  url={https://transparency.entsoe.eu/?site_preference=normal},
  year={2023}
}

@misc{github,
  title={Feature-driven-trading-of-wind-energy-and-hydrogen},
  url={https://github.com/emilhelgren/feature-driven-trading-of-wind-power-and-hydrogen},
  year={2023}
}

@misc{feature_driven,
  doi = {10.48550/ARXIV.1907.07580},
  
  howpublished = {\url{https://arxiv.org/abs/1907.07580}},
  
  author = {Muñoz, Miguel Á. and Morales, Juan M. and Pineda, Salvador},
  
  keywords = {Optimization and Control (math.OC), Applications (stat.AP), Machine Learning (stat.ML), FOS: Mathematics, FOS: Mathematics, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Feature-driven Improvement of Renewable Energy Forecasting and Trading},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{wind_trading_2,  author={Skajaa, Anders and Edlund, Kristian and Morales, Juan M.},  journal={IEEE Transactions on Power Systems},   title={Intraday Trading of Wind Energy},   year={2015},  volume={30},  number={6},  pages={3181-3189},  doi={10.1109/TPWRS.2014.2377219}}

@article{Morales2010,
  title={Short-term trading for a wind power producer},
  author={Morales, JM and Conejo, AJ and P{\'e}rez-Ruiz, J},
  journal={IEEE Transactions on Power Systems},
  volume={25},
  number={1},
  pages={554--564},
  year={2010}
}

@article{pinson2007trading,
  title={Trading wind generation from short-term probabilistic forecasts of wind power},
  author={Pinson, Pierre and Chevallier, Christophe and Kariniotakis, George N},
  journal={IEEE Transactions on Power Systems},
  volume={22},
  number={3},
  pages={1148--1156},
  year={2007},
  publisher={IEEE}
}

@article{conic,
  title={A conic model for electrolyzer scheduling},
  author={Raheli, Enrica and Werner, Yannick and Kazempour, Jalal},
  journal={Computers \& Chemical Engineering},
  volume={179},
  pages={108450},
  year={2023}
}

@article{pinsondro,
  title={Distributionally robust trading strategies for renewable energy producers},
  author={Pinson, Pierre},
  journal={IEEE Transactions on Energy Markets, Policy and Regulation},
  volume={1},
  number={1},
  pages={37--47},
  year={2023},
  publisher={IEEE}
}

@book{xu,
  title={Robust Optimization in Short-Term Power System Operations},
  author={A. Sun and A. J. Conejo},
  year={2021},
  publisher={Springer}
}

@article{bertsimas2019,
  title={From Predictive to Prescriptive Analytics},
  author={Bertsimas, Dimitris and Kallus, Nathan},
  journal={Management Science},
  volume={66},
  number={3},
  pages = {1025--1044},
  year={2019}
}

@article{munoz2020feature,
  title={Feature-driven improvement of renewable energy forecasting and trading},
  author={Mu\~noz, MA and Morales, Juan M and Pineda, Salvador},
  journal={IEEE Transactions on Power Systems},
  volume={35},
  number={5},
  pages={3753--3763},
  year={2020},
  publisher={IEEE}
}

@article{stratigakos2021prescriptive,
  title={Prescriptive Trees for Integrated Forecasting and Optimization Applied in Trading of Renewable Energy},
  author={Stratigakos, Akylas and Camal, Simon and Michiorri, Andrea and Kariniotakis, Georges},
  journal={IEEE Transactions on Power Systems,},
  year={2022},
  volume={37},
  number={6},
  pages = {4696-4708}
}

@misc{PtX_strategy_DK,
    title = {The Goverment's Strategy for Power-to-X},
    year = {2021},
    author = {{Danish Ministry of Climate, Energy and Utilities}},
    pages = {5},
    note ={\url{https://ens.dk/sites/ens.dk/files/ptx/strategy_ptx.pdf}}
}

@misc{RFNBO,
    title = {Delegated act on renewable fuels of non-biological origin},
    year = {2023},
    author = {{European Commission}},
    note ={\url{https://energy.ec.europa.eu/system/files/2020-07/hydrogen_strategy_0.pdf} }
}

@article{liyanage2005practical,
  title={A practical inventory control policy using operational statistics},
  author={Liyanage, Liwan H and Shanthikumar, J. George},
  journal={Operations Research Letters},
  volume={33},
  number={4},
  pages={341--348},
  year={2005}
}

@INPROCEEDINGS{Parginos,
  author={Parginos, Konstantinos and Bessa, Ricardo and Camal, Simon and Kariniotakis, Georges},
  booktitle={2022 IEEE PES Innovative Smart Grid Technologies Conference Europe (ISGT-Europe)}, 
  title={Interpretable data-driven solar power plant trading strategies}, 
  year={2022},
  pages={1-5}
}


@article{sadana2023survey,
  title={A survey of contextual optimization methods for decision making under uncertainty},
  author={Sadana, Utsav and Chenreddy, Abhilash and Delage, Erick and Forel, Alexandre and Frejinger, Emma and Vidal, Thibaut},
  journal={arXiv preprint arXiv:2306.10374},
  year={2023}
}

@article{elmachtoub2022smart,
  title={Smart ''predict, then optimize"},
  author={Elmachtoub, Adam N and Grigas, Paul},
  journal={Management Science},
  volume={68},
  number={1},
  pages={9--26},
  year={2022},
  publisher={INFORMS}
}

==> sections/00.abstract.tex <==
% \section*{Abstract}

